Inferring Accurate Bus Trajectories from Noisy Estimated Arrival Time Records

Urban commuting data has long been a vital source of understanding population mobility behaviour and has been widely adopted for various applications such as transport infrastructure planning and urban anomaly detection. While individual-specific transaction records (such as smart card (tap-in, tap-out) data or taxi trip records) hold a wealth of information, these are often private data available only to the service provider (e.g., taxicab operator). In this work, we explore the utility in harnessing publicly available, albeit noisy, transportation datasets, such as noisy "Estimated Time of Arrival" (ETA) records (commonly available to commuters through transit Apps or electronic signages). We first propose a framework to extract accurate individual bus trajectories from such ETA records, and present results from both a primary city (Singapore) and a secondary city (London) to validate the techniques. Finally, we quantify the upper bound on the spatiotemporal resolution, of the reconstructed trajectory outputs, achieved by our proposed technique.

==> 01-motivation.tex <==
\section{Motivating Scenarios}
The ability to track trajectories of individual buses at real-time lends itself to several \emph{smart city} application scenarios. \kj{not complete yet, needs editing}

\textbf{Event Detection and Forecasting: }Accurate estimations of timings at which individual buses cross respective downstream bus stops allows one to further monitor the occupancy level changes \emph{at} those stops. With longitudinal observations of such fine-grained (i.e., bus stop level), occupancy (or \emph{loading}) level changes, it then becomes possible to (a) curate \emph{expected} or \emph{normal} crowd levels accounting for factors such as day of the week, time of the day, locality, etc., and (b) detect anomalous events where large deviations from such normal patterns are observed, as explored in recent works \cite{xx, yy}. But more importantly, by exploiting the inherent structure of the road network (with several criss-crossing or intersecting bus routes) along with the ability to observe crowd levels at each upstream bus stop, can allow for such anomalies to be \emph{predicted} ahead of time.

\textbf{Predictive Bus Occupancy Monitoring: }Such fine-grained, near real-time, crowd occupancy level change observations can also allow for improvements to current transit Apps that provide ETA and expected occupancy information to passengers waiting for buses to board downstream. For instance, consider a scenario where public commuter Alice is waiting at a bus stop \emph{Station S} and to reach her destination stop \emph{Station D}. She has three choices of services \emph{service1, service2, and service 3} to reach from $S$ to $D$ and her current App informs her that the three services are expected to arrive in \emph{5, 6 and 8} minutes, with crowd levels aboard the incoming bus being \emph{medium, medium, and low}, respectively, and she chooses to wait for $service3$ as it's the least crowded although the waiting time is higher among the alternatives. However, as the bus reaches her stop, she realizes that the crowd level has become higher, as possibly, the bus saw a large amount of passengers boarding at the stop immediately before $S$. However, the ability to 

% \subsection{Opportunities and Challenges}



==> 04b-case.tex <==


\section{Case Study: Event Detection}
% \am{I feel this could be a different section. it's not part of the 'core evaluation'. rather this is an "Illustratve use Case: Event Detection (this de-emphasizes the centrality of event detection)}

% \am{Comparisons include: event detection --(i) based on just bus load level [no dedup, no stitch]; (ii) Delta-occup (dedup-ETA+GPS); (iii) Delta-occup (dedup-ETA only); (iv) Delta-occup (dedup-GPS only) (v) delta-occup (stitching); also analyze at grid-level granularity.}
In this section, we describe our efforts in using crowd level changes \emph{at} bus stops, in the application of detecting events, and in particular, in the discrimination between the start and end of an event. We expect that the start of an event would be less recognizable as the ingress of people to the event would be a slow process whilst the egress would be a more sudden outlet of people from the event venue.

In line with previous works on event detection \cite{XX, YY, ZZ}, we take the case of a single event, ``Britney Spears Live In Concert" that took place in Singapore on June 30th, 2017, and investigate in depth the ability of bus ETA records in detecting such large scale events. We identified XXXX bus stops in the vicinity of the stadium where the event took place, and limit the scope of the evaluation to those. We also note here that the stadium is also accessible by other transportation means -- a Mass Rapid Transit (MRT) station is housed directly under the stadium, is easily accessible by taxis and has ample parking lots for those attending using private vehicles. These, we believe, would reduce the number of the public who might consider bus as their main mode of transport to and fro from the venue.

We resort to $z-score$-based outlier detection techniques similar to the works of XXX \cite{XXX} for detecting the event. We consider the change in occupancy for over every 15 minute interval over the day for all weekdays in June, 2017. We assume that the occupancy changes of each 15 minute window follows the Normal distribution, and compute the $z-$score \cite{XXX}. If the score is greater than a threshold (2.5 in our case), we decide that the particular bus service, at that bus stop, for that time window, is \emph{anomalous}. From the direction of the anomaly, we can further deduce whether the \emph{event} refers to an anomalous amount of people getting in or getting out.

In Figure~\ref{fig:crowd}, we compare the $z-$scores extracted based on (1) raw bus ETA records, (2) after de-duplication and (3) after stitching, for the three bus stops closest by distance to the event venue. The $x-$ axis shows the 5 hour window encapsulating the event hours (i.e., 6 PM to 8 PM), at 15 minute intervals. The $y-$ axis shows the variation in $z-$ score. (per service)(per bus stop)(original plan)

In Figure~\ref{fig:crowd-agg}, we aggregate the occupancy level changes at bus stops at different distances away from the event venue: (1) bus stops within $d$ km, (2) bus stops within XXX km and so on (depicted by the concentric circles in Figure~\ref{fig:concentric}.

We make the following observations:


\begin{figure}[!tbp]
  \centering
  \begin{minipage}[b]{0.4\textwidth}
    \includegraphics[width=\textwidth]{Figs/placeholder.png}
    \caption{Change in crowd level at bus stops near the event venue.}
    \label{fig:crowd}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.4\textwidth}
    \includegraphics[width=\textwidth]{Figs/placeholder.png}
    \caption{Impact on services with increasing distance from the venue.}
     \vspace{-0.2in}
    \label{fig:crowd-agg}
  \end{minipage}
\end{figure}

% \begin{figure}[t]
%     \centering
% 	\includegraphics[width=2in]{Figs/placeholder.png}
% \caption{Change in crowd level at end times of events (against other hours)}
% % \vspace{-0.1in}
% \label{fig:crowd}
% \end{figure}

